Data-driven Coordinated AC/DC Control Strategy for Frequency Safety

With high penetrations of renewable energy and power electronics converters, less predictable operating conditions and strong uncertainties in under-frequency events pose challenges for emergency frequency control (EFC). On the other hand, the fast adjustability of converter-based sources presents opportunities to reduce economic losses from traditional load shedding for EFC. By integrating DC power emergency support, a data-driven coordinated AC/DC control strategy for frequency safety - Coordinated Emergency Frequency Control (CEFC) - has been designed. CEFC coordinates both the initiation and control amount of emergency DC power support (EDCPS) and traditional load shedding. Based on real-time power system response data, CEFC ensures system frequency safety at a minimum control cost under non-envisioned operating conditions and large power deficits. A sufficient condition where data-driven modeling errors do not affect the precision of the control strategy for power system frequency is rigorously provided. Simulation results demonstrate CEFC's adaptability, prediction accuracy, and control effectiveness.

==> gongshi.tex <==
$\boldsymbol{\varepsilon_{\varphi}}$ $\boldsymbol{\varepsilon_{\Lambda}}$

$\boldsymbol{\gamma}(\boldsymbol{x})/\boldsymbol{\boldsymbol{\varphi}}(\boldsymbol{x})$

$\boldsymbol{\beta}(\boldsymbol{x})/\boldsymbol{\boldsymbol{\varphi}}(\boldsymbol{x})$

$\dot{\boldsymbol{\psi}}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})$

$\boldsymbol{\psi}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})$

$\boldsymbol{\beta}^{\text{T}}(\boldsymbol{x})/\boldsymbol{\boldsymbol{\varphi}}^{\text{T}}(\boldsymbol{x})$

$\dot{\boldsymbol{\psi}}^{\text{T}}(\boldsymbol{x})/\boldsymbol{\varphi}^{\text{T}}(\boldsymbol{x})$

$\boldsymbol{\psi}^{\text{T}}(\boldsymbol{x})/\boldsymbol{\varphi}^{\text{T}}(\boldsymbol{x})$

$\textbf{N}\textbf{R}^{-1}\textbf{M}^{\text{T}}$

$\textbf{N}\textbf{R}^{-1}\textbf{N}^{\text{T}}$


$\left\|\boldsymbol{P}\right\|$
$\left\|\boldsymbol{P}\right\|^{2}$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\right\|$ $\left\|\boldsymbol{\varepsilon_{\Lambda}}\right\|$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\right\|^{2}$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\boldsymbol{\varepsilon_{\Lambda}}\right\|$

$\left\|\boldsymbol{\beta}(\boldsymbol{x})/\boldsymbol{\boldsymbol{\varphi}}(\boldsymbol{x})\right\|$

$\left\|\dot{\boldsymbol{\psi}}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$

$\left\|\boldsymbol{\psi}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$

$\left\|\boldsymbol{\Lambda}\boldsymbol{\psi}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$

$\left\|\textbf{M}\textbf{R}^{-1}\textbf{N}^{\text{T}}\right\|$

$\left\|\textbf{M}\textbf{R}^{-1}\textbf{M}^{\text{T}}\right\|$

$\left\|\textbf{N}\textbf{R}^{-1}\textbf{M}^{\text{T}}\right\|$

$\left\|\textbf{N}\textbf{R}^{-1}\textbf{N}^{\text{T}}\right\|$

$\boldsymbol{\varepsilon_{\varphi}}$ $\boldsymbol{\varepsilon_{\Lambda}}$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\right\|^{2}$
$\boldsymbol{\varepsilon}^2_{\boldsymbol{\varphi}}$




$\textbf{N}\textbf{R}^{-1}\textbf{M}^{\text{T}}$

$\textbf{N}\textbf{R}^{-1}\textbf{N}^{\text{T}}$

$\textbf{M}\textbf{R}^{-1}\textbf{M}^{\text{T}}\boldsymbol{P}$

$\textbf{N}\textbf{R}^{-1}\textbf{N}^{\text{T}}\bar{\boldsymbol{P}}$
$\textbf{M}\textbf{R}^{-1}\textbf{N}^{\text{T}}\bar{\boldsymbol{P}}$
$\textbf{N}\textbf{R}^{-1}\textbf{M}^{\text{T}}\bar{\boldsymbol{P}}$

$\bar{\textbf{M}}\textbf{R}^{-1}\bar{\textbf{M}}^{\text{T}}\bar{\boldsymbol{P}}$

$\textbf{M}+\boldsymbol{\varepsilon_{\varphi}}\textbf{N}$

$\mathcal{O}$

$\left\|\boldsymbol{P}\right\|$
$\left\|\boldsymbol{P}\right\|^{2}$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\right\|$ $\left\|\boldsymbol{\varepsilon_{\Lambda}}\right\|$

$\left\|\chi\right\|$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\right\|^{2}$
$\left\|\boldsymbol{\varepsilon_{\varphi}}\boldsymbol{\varepsilon_{\Lambda}}\right\|$

$\left\|\boldsymbol{\beta}(\boldsymbol{x})/\boldsymbol{\boldsymbol{\varphi}}(\boldsymbol{x})\right\|$

$\left\|\dot{\boldsymbol{\psi}}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$

$\left\|\boldsymbol{\psi}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$

$\left\|\boldsymbol{\Lambda}\boldsymbol{\psi}(\boldsymbol{x})/\boldsymbol{\varphi}(\boldsymbol{x})\right\|$
